Event-based Sensor Fusion and Application on Odometry: A Survey

Event cameras, inspired by biological vision, are asynchronous sensors that detect changes in brightness, offering notable advantages in environments characterized by high-speed motion, low lighting, or wide dynamic range. These distinctive properties render event cameras particularly effective for sensor fusion in robotics and computer vision, especially in enhancing traditional visual or LiDAR-inertial odometry. Conventional frame-based cameras suffer from limitations such as motion blur and drift, which can be mitigated by the continuous, low-latency data provided by event cameras. Similarly, LiDAR-based odometry encounters challenges related to the loss of geometric information in environments such as corridors. To address these limitations, unlike the existing event camera-related surveys, this paper presents a comprehensive overview of recent advancements in event-based sensor fusion for odometry applications particularly, investigating fusion strategies that incorporate frame-based cameras, inertial measurement units (IMUs), and LiDAR. The survey critically assesses the contributions of these fusion methods to improving odometry performance in complex environments, while highlighting key applications, and discussing the strengths, limitations, and unresolved challenges. Additionally, it offers insights into potential future research directions to advance event-based sensor fusion for next-generation odometry applications.

==> Sections/04-Experiment.tex <==
\section{Event-based Visual Odometry}~\label{sec:odom}
\red{IN PROGRESS}
% \red{TODO} 
\subsection{Visual Odometry}
\red{Hasier}
\subsection{Event-based Visual Odometry}
\red{Add application chart}
The first event-based pose estimation work was presented by Weikersdorfer et al.~\cite{weikersdorfer2012event} in 2012. This work was extended to an event-based visual SLAM system in 2013~\cite{weikersdorfer2013simultaneous}.

\red{vo}
In 2014, Andrea Censi and Davide Scaramuzza proposed a low-latency event-based visual odometry system~\cite{censi2014low}, which was a significant advancement in reducing the latency associated with traditional frame-based methods. This system utilized asynchronous event data to compute odometry in real-time, paving the way for faster and more efficient pose estimation in dynamic environments. Then in 2016, the work was further enhanced the field by introducing low-latency visual odometry using event-based feature tracks~\cite{kueng2016low}. This method tracked feature points based on event data, achieving reliable and low-latency odometry even in conditions where traditional frame-based methods would struggle, such as in fast motion or poor lighting.
The same group developed a 6-degree-of-freedom (DoF) event-based tracking and mapping system, which relied on geometric principles to perform both parallel tracking and mapping in real time~\cite{rebecq2016evo}. This work was instrumental in showcasing the potential of event cameras for performing full 3D tracking and mapping tasks, marking another milestone in event-based VO.

In 2022, Hidalgo-Carrión et al. proposed event-aided direct sparse odometry (DSO), where event data was combined with traditional direct sparse odometry to improve the robustness of visual odometry in environments with challenging lighting or rapid motion changes~\cite{Hidalgo-Carrio_2022_CVPR}. This method demonstrated the fusion of event-based and frame-based approaches in improving VO performance.


\red{vio}
Integrating an IMU into visual odometry systems significantly enhances their performance by providing additional, reliable motion information that compensates for the limitations of visual data alone. 
In 2017, Zhu et al. extended the capabilities of event-based odometry by integrating inertial measurements in their work on event-based visual-inertial odometry (EVIO)~\cite{Zhu_2017_CVPR}. The combination of event cameras and inertial sensors allowed for robust pose estimation even in challenging scenarios, such as high-speed motion or complex dynamic scenes.
In 2018, Elias Mueggler and his team presented a continuous-time visual-inertial odometry approach for event cameras, further enhancing the accuracy and robustness of event-based odometry systems~\cite{mueggler2018continuous}. Their work highlighted the importance of fusing temporal information from both event data and inertial sensors in a continuous-time framework.

Florian Mahlknecht et al. explored event camera-based odometry for planetary robots in 2022, showcasing the potential of event cameras in extraterrestrial environments where traditional cameras may struggle due to harsh conditions~\cite{mahlknecht2022exploring}.
In 2023, the authors in~\cite{lee2023event} introduced a hybrid approach combining event-and frame-based visual-inertial odometry with adaptive filtering techniques based on 8-DoF warping uncertainty. This method enhanced the odometry system's resilience to noise and dynamic changes, further improving the robustness and adaptability of event-based systems in various application settings.

\subsection{Event-based Stereo Visual Odometry}
Event-based stereo visual odometry is an evolving field that leverages the advantages of stereo event cameras, which provide asynchronous data from two synchronized event sensors, allowing for 3D depth perception in challenging environments with high-speed motion or varying lighting conditions.
The early works on Event-based stereo VO were published in 2018. Henri Rebecq et al.~\cite{rebecq2018emvs} introduced EMVS (Event-based Multi-View Stereo), which enabled 3D reconstruction in real-time using event cameras. This method capitalized on the asynchronous nature of events to compute depth information by fusing event data from multiple viewpoints, enabling accurate and efficient 3D reconstruction. 
In the same year, a semi-dense 3D reconstruction method using stereo event cameras was proposed~\cite{zhou2018semi}. Their approach utilized stereo event cameras to reconstruct semi-dense 3D maps, significantly improving the accuracy and robustness of visual odometry systems, even in dynamic environments.
In~\cite{zhu2018multivehicle}, the authors presented the Multivehicle Stereo Event Camera Dataset, specifically designed for 3D perception. This dataset provided benchmark data for stereo event-based odometry, enabling further research in event-based 3D perception. By providing a large-scale, real-world dataset, this work facilitated the evaluation of stereo event camera systems in various challenging scenarios.

In 2021, Zhou et al.~\cite{zhou2021event} extended their prior work in~\cite{zhou2018semi} by introducing a complete event-based stereo visual odometry system. Their method combined stereo event cameras and a robust odometry pipeline to estimate camera motion in real-time. By leveraging the high temporal resolution of event cameras, this system was able to track fast-moving objects and scenes with challenging lighting conditions.
The feature-based method can also be utilized on event-based stereo visual odometry~\cite{hadviger2021feature}. Their approach detected and tracked features directly from stereo event data, using them to estimate motion. 

Recently, research in stereo event-based visual-inertial odometry (VIO) has gained attention, as it enhances motion estimation by fusing inertial measurements with visual data to improve accuracy and robustness, particularly in conditions where visual information alone may be unreliable.
In 2023, Kunfeng Wang, Kaichun Zhao, and Zheng You developed a stereo event-based visual-inertial odometry (VIO) system, which incorporated both stereo event cameras and inertial measurements to improve the accuracy of pose estimation~\cite{wang2023stereo}.
Further research into stereo event-based VIO led to the work of Peiyu Chen et al.~\cite{chen2023esvio}. 
In parallel, Liu et al. also presented an event-based stereo visual-inertial odometry system~\cite{liu2023esvio}.
Their methods demonstrated superior performance in both accuracy and robustness when compared to frame-based VIO systems, particularly in scenarios involving rapid motion.

Most recent works by Junkai Niu et al. have continued to push the boundaries of event-based stereo VO. Their IMU-aided event-based stereo visual odometry system\cite{niu2024imu} and ESVO2~\cite{niu2024esvo2} incorporate direct visual-inertial odometry with stereo event cameras, significantly improving real-time pose estimation accuracy. These systems integrate IMU data to provide additional motion information, enhancing the overall robustness and accuracy of stereo event-based VIO in complex, real-world environments.

\subsection{\red{Event-based LiDAR Odometry?}}

% https://link.springer.com/chapter/10.1007/978-3-031-72658-3_8
% https://opg.optica.org/abstract.cfm?uri=COSI-2024-CM2B.4

% \begin{figure*}[htbp]
% 	\centering
% 	\begin{minipage}[c]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{Figs/cloud_plot_ape_t01.png}
% 		\subcaption{APE of TB01}
% 		\label{fig:ape_boxplot01}
% 	\end{minipage} 
%          \begin{minipage}[c]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{Figs/cloud_plot_ape_t02.png}
% 		\subcaption{APE of TB02}
% 		\label{fig:ape_boxplot02}
% 	\end{minipage} \\
 
% 	\begin{minipage}[c]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{Figs/cloud_plot_ape_t03.png}
% 		\subcaption{APE of TB03}
% 		\label{fig:ape_boxplot03}
% 	\end{minipage} 
% 	\begin{minipage}[c]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{Figs/cloud_plot_ape_t04.png}
% 		\subcaption{APE of TB04}
% 		\label{fig:ape_boxplot04}
% 	\end{minipage}
% 	\caption{Absolut Positioning Error (APE) of Turtlebot4}
% 	\label{fig:ape_boxplot}
% \end{figure*}

% \begin{figure*}[htbp]
% 	\centering
% 	\begin{minipage}[c]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{Figs/clip45to125cloud_plot_ape_t01.png}
% 		\subcaption{APE of TB01}
% 		\label{fig:ape_boxplot01}
% 	\end{minipage} 
%          \begin{minipage}[c]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{Figs/clip45to125cloud_plot_ape_t02.png}
% 		\subcaption{APE of TB02}
% 		\label{fig:ape_boxplot02}
% 	\end{minipage} \\
 
% 	\begin{minipage}[c]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{Figs/clip45to125cloud_plot_ape_t03.png}
% 		\subcaption{APE of TB03}
% 		\label{fig:ape_boxplot03}
% 	\end{minipage} 
% 	\begin{minipage}[c]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{Figs/clip45to125cloud_plot_ape_t04.png}
% 		\subcaption{APE of TB04}
% 		\label{fig:ape_boxplot04}
% 	\end{minipage}
% 	\caption{Absolut Positioning Error (APE) of Turtlebot4}
% 	\label{fig:ape_boxplot}
% \end{figure*}

% \begin{table}[h]
%     \centering
%     \caption{RMSE\/STD Results}
%     \label{tab:RMSE_STD}
%     \begin{tabular}{@{}lccccl@{}}
%     \toprule
%     \textbf{ } & \textbf{Scenarios} & \textbf{RMSE} & \textbf{STD} \\ 
%     \midrule
%     TB01 & ALL       & 0.122  &  0.064  \\
%     TB01 & ALL       & 0.122  &  0.064  \\
%     TB01 & ALL       & 0.122  &  0.064  \\
%     TB01 & ALL       & 0.122  &  0.064  \\
%     TB01 & ALL       & 0.122  &  0.064  \\
%     TB01 & ALL       & 0.122  &  0.064  \\
%     TB01 & ALL       & 0.122  &  0.064  \\
%     % Without security & 72.11 ms    &   9804 bytes/sec &  0.06 \% \\ 
%     \bottomrule
%     \end{tabular}
% \end{table}



